Predicting Out-of-Domain Generalization with Neighborhood Invariance

Developing and deploying machine learning models safely depends on the ability to characterize and compare their abilities to generalize to new environments. Although recent work has proposed a variety of methods that can directly predict or theoretically bound the generalization capacity of a model, they rely on strong assumptions such as matching train/test distributions and access to model gradients. In order to characterize generalization when these assumptions are not satisfied, we propose neighborhood invariance, a measure of a classifier's output invariance in a local transformation neighborhood. Specifically, we sample a set of transformations and given an input test point, calculate the invariance as the largest fraction of transformed points classified into the same class. Crucially, our measure is simple to calculate, does not depend on the test point's true label, makes no assumptions about the data distribution or model, and can be applied even in out-of-domain (OOD) settings where existing methods cannot, requiring only selecting a set of appropriate data transformations. In experiments on robustness benchmarks in image classification, sentiment analysis, and natural language inference, we demonstrate a strong and robust correlation between our neighborhood invariance measure and actual OOD generalization on over 4,600 models evaluated on over 100 unique train/test domain pairs.

==> extra_tables.tex <==
\begin{subtable}{1\textwidth}
\centering
\small
\begin{tabular}{lccccc}
\toprule
& \multicolumn{5}{c}{Train Domain (Model)}\\
\cmidrule{2-6}
Measure & SVHN (NiN) & CIFAR10 (NiN) & CIFAR10 (VGG) & CIFAR10 (ResNet) & CINIC10 (CNN)\\
\midrule
NI-RandAug & 0.648 & 0.464 & 0.594 & 0.373 & \textbf{0.664} \\
NI-Rotate & & & & & \\
NI-Erase & 0.463 & 0.189 & 0.583 & 0.296 & 0.662\\
NI-FC & 0.426 & 0.578 & \textbf{0.663} & 0.534 & \textbf{0.664}\\
\midrule
ATC-NE & 0.722  & \textbf{0.631} & 0.584 & 0.551 & 0.662 \\
ATC-MC & \textbf{0.741} & 0.610 & 0.592 & \textbf{0.577} & 0.660 \\
\bottomrule
\end{tabular}
\caption{Results on image classification tasks.}
\label{tab:app_full_idt_cnn_aws}
\vspace{0.5cm}
\end{subtable}

==> old_related.tex <==
%\subsection{Measuring Function Smoothness}
\textbf{Measuring Model Invariance and Smoothness} \quad
Enforcing various kinds of model invariance \citep{zhu2021understanding} has been shown to improve generalization, including invariance to data augmentations \citep{cubuk2020randaugment} and invariance to linear interpolations between points \citep{zhang2018mixup}.
The notion of invariance that we define in our work is also related to notions of function smoothness.
The simplest way to measure the smoothness of a function $f:\mathcal{X} \rightarrow \mathcal{Y}$ is through its differentiability class. 
However, this is not a very useful inductive bias for a model since differentiability is local and metric dependent.
One alternative measure is Lipschitz continuity. 
Enforcing this property on neural networks is commonly done by restricting the learned function class with spectral regularization \citep{yoshida2017spectral}, spectral normalization \citep{takeru2018spectral}, and other norm based regularization methods on layer weights \citep{bartlett2017spectrally, neyshabur2017exploring, foret2020sharpness}.
Other methods regularize the the norm of gradients with respect to the the inputs of the network \citep{elsayed2018large, arbel2018gradient,gulrajani2017improved}.
A key component of smoothness regularization is \textit{where} and \textit{how} it is enforced. 
Enforcing global properties such as Lipschitz continuity in regions where there is no data can restrict the learned function unnecessarily \citep{rosca2020case}.
%In addition, if the data lies on a low-dimensional manifold, then smoothness should only be regularized with respect to this manifold, rather than the entire space.

\textbf{Intrinsic Dimensionality and Neighborhood Regularization} \quad
Recent work has proven estimation error bounds for deep ReLU networks in H{\"o}lder\citep{schmidt2019deep, ryumei2020adaptive,chen2019nonparametric}, Besov, mixed smooth Besov\citep{suzuki2018adaptivity}, and anisotropic Besov \citep{suzuki2021deep} function spaces based on their intrinsic dimensionality and smoothness.
However, it is still unclear how to measure the intrinsic dimensionality or smoothness of functions on complex manifold spaces.
Separate work aims to model local neighborhoods rather than the entire manifold space
 by encouraging invariance to local changes \citep{rifai2011manifold}, augmentation graphs \citep{haochen2021provable}, similar neighbors \citep{luo2018smooth}, or interpolation between points \citep{chaudhuri2019manifold}.

==> old_toy.tex <==
\addplot+[blue, mark options={blue}] table [x=x, y=y, col sep=comma] {
x,  y
1,0.684507570926505,0.7427210349440576,0.08876675212289717,0.9670397000000002,0.008357018922258482
2,0.6511945941173707,0.7374680342078209,0.08906259593370974,0.9683885999999999,0.00763540691881393
3,0.593170759262823,0.7301460340619087,0.08695303657328932,0.9703231999999999,0.007435493111040542
4,0.4746651994584562,0.7150930339694023,0.09004184462803022,0.9732113,0.007428918756370561
5,0.36778692856735057,0.7001700337529182,0.08990269145281495,0.9754346999999999,0.007597146324754675
6,0.2642113273911152,0.6772500317394734,0.09357556926267167,0.9785960000000001,0.008674983718633938
7,0.249938681994345,0.6684960312843323,0.10511744153473239,0.9807070000000001,0.00892236178477062
8,0.18317503146173672,0.6477860294878482,0.1188573768989026,0.9842583000000001,0.009638501377346793
9,0.1329060915819386,0.6287990294694901,0.1268627052725788,0.9840287,0.009615889643311237
10,0.08641056788793153,0.614638028383255,0.13145291143512552,0.9864067999999999,0.009839043097721522
11,0.07513682062918896,0.6105280293524266,0.13044856863801554,0.9872428000000001,0.009647476772677448
12,0.020659000826420852,0.5733590268492699,0.15579098575361527,0.987344,0.009895639307268934
13,0.042529917734954646,0.5898900273740292,0.13854878377900537,0.9939059840000001,0.00536688161544307
14,0.004430022305175849,0.5677660254836082,0.1620107502709051,0.994213784,0.005244474787024923
15,-0.0649106350220563,0.558228025496006,0.1585012656597681,0.9944405599999999,0.0052409372337472926
16,-0.08457184095805173,0.5461650254428386,0.1647104913603199,0.9946889599999998,0.005169752028342667
17,-0.09380251456627395,0.5464930244684221,0.17043036868700948,0.9952619599999999,0.005022091402505761
18,-0.17494423912188667,0.5221070238649845,0.17462019287284913,0.9952536000000001,0.005106775930037849
19,-0.3253734127465416,0.49425902262330057,0.17150972325490307,0.995329564,0.005128074097663299
20,-0.2365407209619934,0.5070340220630168,0.17378395679402084,0.9953363239999999,0.00521163606781796
21,-0.2950146170556473,0.48514102306962015,0.1835013768442912,0.995590844,0.005001714545955485
22,-0.3660877044132819,0.4718020226359368,0.17992783902811377,0.995895516,0.005073804359758114
23,-0.40161414116194605,0.46405502223968503,0.17163410321929257,0.995674232,0.005091620966501262
24,-0.4131779302395805,0.46777002105116844,0.1668040280983026,0.9958619760000001,0.004913339971006623
25,-0.4771593316953669,0.44236302316188814,0.17369666639106968,0.996051192,0.004968647157914707
26,-0.5049008693376914,0.4440860199034214,0.1623418255287009,0.996008636,0.004896417039619556
27,-0.6010528630423656,0.4157970193326473,0.15769859445355522,0.99645906,0.004863176713929168
28,-0.6051552304800824,0.4189620192050934,0.1485263729232631,0.996038332,0.005070713073952546
29,-0.6526385651189951,0.40060001924633976,0.1424550642668671,0.996549048,0.004879466157831334
30,-0.6567647932797176,0.39607501843571663,0.1448314616606957,0.99667496,0.004848685719262754
31,-0.6674950253949886,0.3933990183472633,0.14555568253893916,0.996552904,0.004867502359127489
32,-0.7335482572658847,0.3758940227925778,0.1330627964135444,0.997011284,0.004602375323590124
33,-0.7521783993470279,0.3742630177140236,0.11416758572495707,0.99729306,0.004372315735491919
34,-0.7860468206375615,0.3575830196142197,0.11508802859185248,0.997421196,0.004406425777065777
35,-0.7669152517448782,0.3549730171263218,0.11068889395149532,0.9978819800000001,0.004040224366853777
36,-0.7890543861826147,0.34356701731681827,0.11035292493128224,0.9979967399999999,0.004019873647604659
37,-0.746847466408944,0.3508220157623291,0.10295071840590722,0.998052708,0.003944084437431166
38,-0.7618842705158722,0.3377570118606091,0.10254031115566194,0.998145328,0.0040097022907753495
39,-0.7226205769236791,0.33852001786231994,0.09958847713372539,0.9983429559999999,0.0036650992229705164
40,-0.7599846564912213,0.3396360144019127,0.09676888371459362,0.9984684359999999,0.0035326843185554276
};

\begin{figure}[t]
\centering
\begin{tikzpicture}
  %\shade[ball color = gray!40, opacity = 0.2] (0,0) circle (2cm);
  \draw (0,0) circle (2cm);
  \draw (0,0) circle (2cm);
  \draw (-2,0) arc (180:360:2 and 0.4);
  \draw[dashed] (2,0) arc (0:180:2 and 0.4);
  %\fill[fill=black] (0,0) circle (1pt);

  \shade[ball color = gray!40, opacity = 0.4] (0,2cm) circle (0.4cm);
  %\draw (-0.4cm,2cm) arc (180:360:0.4 and 0.1);
  %\draw[dashed] (0.4cm,2cm) arc (0:180:0.4 and 0.1);
  \fill[fill=black] (0,2cm) circle (1.5pt);
    \node[label=above:{$\D_0$}] at (0,2) {};

  %\draw (1,1.73) circle (0.5cm);
  %\draw (0.5,1.74) arc (180:360:0.5 and 0.15);
  %\draw[dashed] (1.5,1.74) arc (0:180:0.5 and 0.15);
  \shade[ball color = gray!40, opacity = 0.4] (-0.6,1.62cm) circle (0.4cm);
  \fill[fill=black] (-0.6,1.62) circle (1.5pt);
  \draw (-1,1.73) arc (180:360:1 and 0.15);
  \draw[dashed] (1,1.73) arc (0:180:1 and 0.15);
      \node[label=left:{$\D_1$}] at (-1,1.73) {};

  %\draw (1.74,1) circle (0.5cm);
  %\draw (1.24,1) arc (180:360:0.5 and 0.15);
  %\draw[dashed] (2.24,1) arc (0:180:0.5 and 0.15);
  %\fill[fill=black] (1.74,1) circle (1pt);
  \shade[ball color = gray!40, opacity = 0.4] (1.1,0.78) circle (0.4cm);
  \fill[fill=black] (1.1,0.78) circle (1.5pt);
  \draw (-1.74,1) arc (180:360:1.74 and 0.3);
  \draw[dashed] (1.74,1) arc (0:180:1.74 and 0.3);
      \node[label=left:{$\D_2$}] at (-1.73,1) {};

  %\draw (2,0) circle (0.5cm);
  %\draw (1.5,0) arc (180:360:0.5 and 0.15);
  %\draw[dashed] (2.5cm,0) arc (0:180:0.5 and 0.15);
  %\fill[fill=black] (2cm,0) circle (1pt);
  \shade[ball color = gray!40, opacity = 0.4] (0.2,-0.38) circle (0.4cm);
  \fill[fill=black] (0.2,-0.38) circle (1.5pt);
    \node[label=left:{$\D_3$}] at (-2,0) {};

  %\draw (1,-1.73) circle (0.5cm);
  %\draw (0.5,-1.74) arc (180:360:0.5 and 0.15);
  %\draw[dashed] (1.5,-1.74) arc (0:180:0.5 and 0.15);
  %\fill[fill=black] (1,-1.73) circle (1pt);
  \draw (-1,-1.73) arc (180:360:1 and 0.15);
  \draw[dashed] (1,-1.73) arc (0:180:1 and 0.1);
    \node[label=left:{$\D_5$}] at (-1,-1.73) {};

  %\draw (1.74,-1) circle (0.5cm);
  %\draw (1.24,-1) arc (180:360:0.5 and 0.15);
  %\draw[dashed] (2.24,-1) arc (0:180:0.5 and 0.15);
  %\fill[fill=black] (1.74,-1) circle (1pt);
  \draw (-1.74,-1) arc (180:360:1.74 and 0.3);
  \draw[dashed] (1.74,-1) arc (0:180:1.74 and 0.3);
    \shade[ball color = gray!40, opacity = 0.4] (-0.5,-1.29) circle (0.4cm);
  \fill[fill=black] (-0.5,-1.29) circle (1.5pt);
  \node[label=left:{$\D_4$}] at (-1.74,-1) {};

  \shade[ball color = gray!40, opacity = 0.4] (0.1,-1.87) circle (0.4cm);
  \fill[fill=black] (0.1,-1.87) circle (1.5pt);


  %\draw (0,-2cm) circle (0.5cm);
  %\draw (-0.5cm,-2cm) arc (180:360:0.5 and 0.15);
  %\draw[dashed] (0.5cm,-2cm) arc (0:180:0.5 and 0.15);
  %\fill[fill=black] (0,-2cm) circle (1pt);
  %\draw[dashed] (0,0 ) -- node[above]{1} (2,0);
\end{tikzpicture}
\caption{We generate data from univariate gaussians whose means lie on a unit hypersphere and train models to classify points as inside or outside this hypersphere. Training data $\D_0$ is centered at a pole and we
consider out-of-domain data regions $\D_j$ that lie along equally spaced circumferences. 
We randomly select points along each circumference and generate a dataset at each point.
We then calculate the correlation between the neighborhood invariance and generalization of our trained models on these datasets.}
\label{fig:measure_graph}
\end{figure}

\begin{figure}
\centering
\begin{tikzpicture}[scale=0.85, trim axis left]
\begin{axis}[
    xlabel=Dataset Distance,
    ylabel=Kendall $\tau$,
    xtick pos=left,
    ytick pos=left,
    ymajorgrids=true,
    xmin=0,xmax=40,
    ymin=-1,ymax=1,
    legend pos=north east,
    height=6cm, width=6.5cm,
    xtick={0,10,20,30,40},
    xticklabels={0,$\pi/4$,$\pi/2$,$3\pi/4$,$\pi$}
    % for log axes, x filter operates on LOGS.
    % and log(x * 1000) = log(x) + log(1000):
    %x filter/.code=\pgfmathparse{#1 + 6.90775527898214},
]

%\addplot[mark=none, black, dashed, ultra thick, samples=4] {66.59};
%\addlegendentry{Baseline}

\addplot+[blue, mark options={blue}, mark size=1pt] table [x=x, y=y, col sep=comma] {
x, y
1,0.6525258532135789
2,0.5830753611787677
3,0.45543136953204966
4,0.3744321562149508
5,0.24657020219981124
6,0.16553698718211124
7,0.18565558926256362
8,0.19396307244029426
9,0.1364864439973082
10,0.03217010429856841
11,-0.012303735318492073
12,-0.03894219069435641
13,-0.01939445522468155
14,-0.08266358111144798
15,-0.03717861509776703
16,-0.13671343303864053
17,-0.1498124792646949
18,-0.2525740586689544
19,-0.28645503604304184
20,-0.32779990005381376
21,-0.29375629068200576
22,-0.3841272995754502
23,-0.36904584564920917
24,-0.37700072347301167
25,-0.4797002655215846
26,-0.46268958172504415
27,-0.5603306585380293
28,-0.5969839914629598
29,-0.5709959115485879
30,-0.6489042029453421
31,-0.6344588008283127
32,-0.6987639382996471
33,-0.7376043095802051
34,-0.7287478253359547
35,-0.739928694083101
36,-0.7558163977982721
37,-0.7318418788241242
38,-0.7576083242534059
39,-0.7664748771610461
40,-0.7269193211206649
};
\addlegendentry{NI}

\addplot+[red, mark=*, mark options={red}, mark size=1pt] table [x=x, y=y, col sep=comma] {
x,y
1,0.6176152287658037
2,0.5368563095778853
3,0.4261757336977026
4,0.31839032830471503
5,0.20612708238947558
6,0.09219225239811502
7,0.0949683718931356
8,0.1254607355949024
9,0.09078205362121733
10,0.02296657018928826
11,-0.03256325454538281
12,-0.04471917424987253
13,-0.032525174088703236
14,-0.06631935206519064
15,-0.0321232932609765
16,-0.13783610157635465
17,-0.14547467271276174
18,-0.22295090869069356
19,-0.27228480132059085
20,-0.31673951851741206
21,-0.27785419674412337
22,-0.3833009737092
23,-0.349260825079429
24,-0.35041238425906446
25,-0.44590152768199937
26,-0.42989184610688075
27,-0.5313357981495975
28,-0.5518072452257601
29,-0.5352931454008542
30,-0.6094983229875618
31,-0.602507277250487
32,-0.6539660615227365
33,-0.672656153785861
34,-0.6746579716954092
35,-0.6759466666310082
36,-0.6779893923608891
37,-0.6804479454039745
38,-0.6900451202848992
39,-0.7030530208638897
40,-0.6769555883215527
};
\addlegendentry{ATC};

\end{axis}
\end{tikzpicture}
\caption{The correlation between neighborhood invariance and OOD generalization remains high for datasets closest to the training domain. As dataset distance increases, correlation quickly decreases, becoming negatively correlated for datasets further than $\pi/4$ away on the hypersphere. We observe the same behavior regardless of the method chosen to predict OOD generalization.}
\label{fig:toy_res}
\end{figure}
